Constant-Time Predictive Distributions for Gaussian Processes

One of the most compelling features of Gaussian process (GP) regression is its ability to provide well-calibrated posterior distributions. Recent advances in inducing point methods have sped up GP marginal likelihood and posterior mean computations, leaving posterior covariance estimation and sampling as the remaining computational bottlenecks. In this paper we address these shortcomings by using the Lanczos algorithm to rapidly approximate the predictive covariance matrix. Our approach, which we refer to as LOVE (LanczOs Variance Estimates), substantially improves time and space complexity. In our experiments, LOVE computes covariances up to 2,000 times faster and draws samples 18,000 times faster than existing methods, all without sacrificing accuracy.

==> results/airline_results.tex <==
\begin{tabular}{ |c|c|c|c| }
  \hline
  \thead{\bf Standard GP}
  &\thead{\bf KISS-GP}
  &\thead{\bf SGPR}
  &\thead{\bf \methodname{}}
  \\
  \hline

  $-221$
  & $-222$
  & $-223$
  & $-222$
  \\
  \hline
\end{tabular}


==> sections/gp_background.tex <==
In this section, we briefly review the fundamentals of Gaussian processes as used for regression in machine learning.
For a full overview, we refer the reader to \cite{rasmussen2006gaussian}.
A Gaussian process is an extension of the multivariate normal distribution to a distribution over real-valued \emph{functions}, $f(\mathbf{x})$, rather than discrete vectors.
Analogous to the mean vector and covariance matrix of a multivariate normal distribution, a Gaussian process is parameterized by a
\emph{mean function} $\mu(\x)$ and a prior \emph{covariance function} $k(\x, \x')$: $f(\x)\sim\mathcal{GP} \left(\mu(\x),k(\x,\x')\right)$.
The marginal distribution of the function values at any finite set of inputs $[\x_{1},...,\x_{n}]$ are jointly Gaussian distributed:
%
\begin{equation}
    \fn = [f(\x_{1}),...,f(\x_{n})]^{\top} \sim\mathcal{N} \left( \mu_{\X}, \K_{\X\X} \right)\nonumber
\end{equation}
%
where $\mu_{\X} \!=\! [\mu(\x_{1}),...,\mu(\x_{n})]^{\top}$ and $\K_{\X\X}\!=\![k(\x_{i},\x_{j})]_{i,j=1}^{n}$.
Generally, $K_{AB}$ denotes a matrix of cross-covariances between the sets $A$ and $B$.
%Throughout, we will denote by $\K_{\A\B}$ the kernel matrix achieved by applying the covariance function to all pairs of points with one from $\A$ and one from $\B$, $(\mathbf{a}_{i}, \mathbf{b}_{j})$. In the case where $\A=\B$, $\K$ is symmetric positive definite.

%It is common in Gaussian process regression to assume an additive noise model relating function values to observed measurements. That is, we assume a weight measurement $y_{i}$ is related to the observed features $\x_{i}$ according to $y_{i}=f(\x_{i}) + \epsilon$, where $\epsilon \sim \mathcal{N} \left(0, \sigma^{2}\right)$.

Under a Gaussian noise observation model,
\[
  p(y(\x) \! \mid \! f(\x)) \sim \mathcal{N}(y(\x); f(\x),\sigma^2),
\]
the posterior $p(f(\x) \posterior)$ conditioned on some data $\mathcal{D} = (X, \y) = \{(\x_i, y_i)\}_{i=1}^{n}$ is again a Gaussian process with mean $\mu_{f \mid \dset}(\x^*)$ and covariance $k_{f \mid \dset}(\x^*,\x^{*\prime})$:
\begin{align}
  %p(f(\x)\posterior) &\sim \mathcal{GP} \left(\mu_{f \mid \dset}(\x), k_{f \mid \dset}(\x, \x')\right), \notag \\
  \mu_{f \mid \dset}(\x^*) &= \mu(\x^*) + \bk_{\X \x^*}^\top  \widehat K_{\X\!\X}^{-1} (\y - \mu(\X)) \label{eq:pred_mean}, \\
  k_{f\mid\dset}(\x^*, \x^{*\prime}) &= k_{\x^{*} \x^{*\prime}} - \bk_{\X \x^{*}}^\top \widehat K_{\X\!\X}^{-1} \bk_{\X \x^{*\prime}},
    \label{eq:pred_covar}
\end{align}
where $\hat{K}_{\X\X} = K_{\X\X} + \sigma^2 I$ and $\y = [y(\x_1),\dots,y(\x_n)]^{\top}$. Given a test point $\x^{*}$, the posterior can be used to make predictions by computing $p(f(\x^{*})\posterior)$ using the equations above. More generally, given a set of $t$ test points $\X^{*}$, the equations above give rise to a $t$ dimensional multivariate Gaussian joint distribution
$p([f(\x^{*}_{1}),...,f(\x^{*}_{t}))]\posterior)$ over the function values of the $t$ test points. This last property allows for sampling functions from a posterior Gaussian process by sampling from this joint predictive distribution.

